Overprotective Training Environments Fall Short at Testing Time: Let Models Contribute to Their Own Training

Despite important progress, conversational systems often generate dialogues that sound unnatural to humans. We conjecture that the reason lies in their different training and testing conditions: agents are trained in a controlled "lab" setting but tested in the "wild". During training, they learn to generate an utterance given the human dialogue history. On the other hand, during testing, they must interact with each other, and hence deal with noisy data. We propose to fill this gap by training the model with mixed batches containing both samples of human and machine-generated dialogues. We assess the validity of the proposed method on GuessWhat?!, a visual referential game.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}


\begin{table*}[t]
	\centering
		\begin{tabular}{|c|c|c|c?c|c|c|c|c|}
		\hline
		\multicolumn{4}{|c?}{\textbf{Training Set}}                                                                                                                                                                                                     & \multicolumn{5}{c|}{\textbf{Test Set - 5Q setting}}                                \\ \hline
		\textbf{\begin{tabular}[c]{@{}c@{}}\% Human \\ Dialogues\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% Generated \\ Dialogues\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generated Dial. \\ Length\end{tabular}} & \textbf{GRQ} & \textbf{ACC$\uparrow$} & \textbf{GRQ$\downarrow$} & \textbf{MO$\downarrow$} & \textbf{NQ$\uparrow$} & \textbf{GR$\uparrow$} \\ \hline
		100                                                                    & 0                                                                          & -                                                                          & 0            & 46.3              & 36.8         & 0.27        & 0.53        & 20.6        \\ \hline
		75                                                                     & 25                                                                         & fixed                                                                  & 2.9          & 47.9              & 24.0           & 0.20        & 0.43        & 20.2        \\ \hline
		75                                                                     & 25                                                                         & variable                                                       & 2.6          & 47.5              & 26.6         & 0.21        & 0.41        & 19.4        \\ \hline
		50                                                                     & 50                                                                         & fixed                                                                 & 5.4          & 48.1              & 22.5         & 0.18        & 0.37        & 21.2        \\ \hline
		50                                                                     & 50                                                                         & variable                                                       & 4.7          & 47.0                & 21.0         & 0.18        & 0.42        & 21.1        \\ \hline
	\end{tabular}
\label{tab_results}
	\caption{GDSE-SL results on several training sets. At test time, the model generates 5 questions and then it guesses. Length ``fixed": 5-turns dialogues. Length ``variable": same turns human annotators used for that game. ACC: accuracy. GRQ: \% games with at least one repeated question. MO: Mutual Overlap. NQ: Novel Questions. GR: Global Recall. $\uparrow$: higher is better. $\downarrow$: lower is better.}
\vspace*{-10pt}
\end{table*}


\cut{We are interested in studying how modifying part of the data in the training set of the GDSE model affects the linguistic output and the model's accuracy of the GuessWhat game. More specifically, we aim at building a training set in which part of the dialogues collected with human annotators are replaced with dialogues generated by the GDSE questioner model while playing with the baseline Oracle model on the same games being replaced. In this way, we build a training set containing dialogues that are more similar to the ones the model will generate at test time. %We conjecture that a model exposed to a small number of ``imperfect" data at training time will less likely get stuck in repetition loops at test time. 
}
As a first step, we trained GDSE for 100 epochs as described in Shekhar et al., \shortcite{shekhar-etal-2019-beyond}. At the end of the training, we used GDSE to play the game with the Oracle on the whole training set, saving all the dialogues. We generate these dialogues with the model trained for all the 100 epochs since it generates fewer repetitions, although it is not the best-performing on the validation set. The dialogues generated by GDSE while playing with the Oracle are noisy: the may contain duplicated questions, wrong answers, etc. See Figure \ref{fig:intro} for an example of human and machine-generated dialogues for the same game.

\cut{Secondly, we built new training sets according to two criteria: the proportion of human and machine-generated data (50-50 or 75-25) and the length of the generated dialogue. Either we always keep a fixed dialogue length (5 turns, as the average length in the dataset) or we take the same number of turns that the human Questioner used while playing the game we are replacing.}

%with different percentages of human dialogues (75\%, 50\%), while the renaming part consists of the dialogues resulting from the previous step. While taking the machine-generated dialogues, we considered two scenarios: one in which we always keep a fixed dialogue length (5 turns, as the average length in the dataset) and another in which we take the same number of turns that the human Questioner used while playing the game we are replacing.

Finally, GDSE is trained again from scratch on these new training sets that are composed of both human and machine-generated dialogues. Note that the model receives batches composed of both human and machine-generated dialogues.


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{figure}[t]\centering 
	\includegraphics[width=0.95\linewidth]{Fig_intro_2.pdf}
	\caption{Two-steps training method.}\label{fig:intro_2}
\end{figure}

\begin{figure*}[t]\centering %\hspace*{-0.1cm}
	\includegraphics[width=0.97\linewidth]{humans_vs_machines.pdf}
	\caption{GuessWhat sample dialogues between two human annotators (left) and two neural conversational agents (right, generated by Shekhar et al. \shortcite{shekhar-etal-2019-beyond}). The yellow box highlights the target entity that the Questioner has to guess by asking binary questions to the Oracle. Note that the dialogue on the right contains repetitions from the Questioner and wrong answers from the Oracle.}\label{fig:intro}
\end{figure*}


Several dialogue tasks have been recently proposed as referential guessing games in which an agent (the Questioner) asks questions to another agent (the Answerer/Oracle) in order to guess the referent entity (e.g. a specific object depicted in an image) they have been speaking about \cite{visdial_rl,guesswhat_game,he:lear17,haber-etal-2019-photobook,ilinykh-etal-2019-tell,udag19}. 
These referential games are usually evaluated by looking at the task success metric, i.e. whether the Questioner is able to correctly identify the referent at the end of a dialogue exchanged with the other agent. 
This simple task success metric, however, does not evaluate a core aspect of these systems, i.e. the linguistic quality of the generated output. The need of going beyond the task success metric has been highlighted in Shekhar et al. \shortcite{shekhar-etal-2019-beyond}, where the authors presented a new state-of-the-art model (GDSE) for the GuessWhat Questioner agent \cite{guesswhat_game} and compare the quality of the dialogues generated by different questioner models according to some linguistic metrics. One striking feature of the dialogues generated by the GDSE model is the large number of games containing repeated questions, while the dialogues used to train the model (collected with human annotators) do not contain repetitions. The GDSE architecture has been recently extended with a "Decider" module \cite{shekhar2019jointly} to stop the dialogue when the agent has gathered enough information, without choosing a priori a fixed number of turns to be generated. This approach is effective in reducing repetitions but, crucially, the task accuracy of the game decreases. 
%A recent paper \cite{shekhar2019jointly} propose to plug a "Decider" module into the GDSE architecture so that the model can decide to stop the dialogue when it has gathered enough information, without choosing a priori a fixed number of turns to be generated before guessing. This approach is effective in reducing repetitions at test time but, crucially, the accuracy on the guessing game decreases. 
Murahari et al. \shortcite{mura:impr19} propose a Questioner model for the GuessWhich task \cite{visdial_rl} that specifically aims to improve the diversity of generated dialogues by adding a new loss function during training: although this technique reduces the number of repeated questions compared to the baseline model, there is still a large number of repetitions in the output. 

The problem of generating repetitions not only affects dialogue systems but instead it seems to be a general property of current decoding strategies. Holtzman et al. \shortcite{holt:cur19} found that decoding strategies that optimize for an output with high probability, such as the widely used beam/greedy search, lead to a linguistic output that is incredibly degenerate. Although language models generally assign high probabilities to well-formed text, the highest scores for longer texts are often repetitive and incoherent. To address this issue, the authors propose a new decoding strategy (Nucleus Sampling) that shows promising results. Our preliminary experiments (not reported in the paper) show that applying Nucleus Sampling as a decoding strategy for GDSE \cite{shekhar-etal-2019-beyond} effectively reduces the number of repetitions, but it leads to awkward dialogues discussing entities that are not present in the visual input, thus dramatically reducing the task success of the game. 

In this paper, we take a step back and explore a simple approach in order to improve the quality of the dialogues generated by the GDSE model \cite{shekhar-etal-2019-beyond} for the GuessWhat game.
Our work is inspired by Sankar et al. \shortcite{sank:done19}, who experiment
with different types of perturbations on multi-turn dialogue datasets: the authors found that generative neural dialogue systems are not significantly affected even by drastic and unnatural modifications to the dialogue history. Unlike Sankar et al. \shortcite{sank:done19}, we do not perturb the training set to scramble the conversational structure but instead we change the nature of the training data. 
We hypothesize that one of the reasons why computational models get stuck in repetition loops while generating natural language could be that they have never seen repetitions at training time. Indeed, human dialogues do not contain repetitions.
Although it may sound counter-intuitive, we hypothesize that models may benefit from seeing at training time data that are more similar to the ones the model can generate, i.e. dialogues with repetitions, wrong answers from the other agent, etc.  In our experiments, we train the GDSE model on a training set in which part of the original GuessWhat dialogues are replaced with the ``noisy" dialogues (see the example in Figure \ref{fig:intro}) generated by the GDSE questioner in Shekhar et al. \shortcite{shekhar-etal-2019-beyond}. Surprisingly, our results show that the Questioner trained on this ``mixed" training set outperforms the model trained on the ``official" training set with respect both to the quality of the linguistic output and the task success in the GuessWhat game. 


==> task_data.tex <==
\section{Dataset and Model}
\label{sec:task_data}

The GuessWhat?! game (de Vries et al. 2017) is a referential communication task where two players collaborate to identify a referent. This setting has been extensively used in human-human collaborative dialogue \cite{clark1996using,yule2013referential}. The GuessWhat?! dataset was collected via Amazon Mechanical Turk by de Vries et al. (2017). It is an asymmetric game involving two human participants who see a real-world image taken from the MS-COCO dataset \cite{lin:micr14}. One of the participants (the Oracle) is secretly assigned a target object within the image and the other participant (the Questioner) has to guess it by asking binary (Yes/No) questions to the Oracle. Humans could stop asking questions at any time, so the length of the dialogues is not fixed. 
%Each game has at least 3 and at most 20 candidates. The dataset contains 155K English dialogues about approximately 66K different images. 
The training set contains about 108K datapoints and the validation and test sets 23K each. Dialogues contain on average 5.2 turns.

In our experiments, we use the Visually-Grounded State Encoder (GDSE)
model of Shekhar et al. \shortcite{shekhar-etal-2019-beyond}, i.e. a
Questioner agent for the GuessWhat?! game. We consider the version of
GDSE trained in a supervised learning fashion (GDSE-SL). The model
uses a visually grounded dialogue state that takes the visual features
of the input image and each question-answer pair in the dialogue
history to create a shared representation used both for generating a
follow-up question (QGen module) and guessing the target object
(Guesser module) in a multi-task learning scenario. The QGen component
is optimized with the Log Likelihood of the training dialogues, and
the Guesser computes a score for each candidate object by performing
the dot product between visually grounded dialogue state and each
object representation. As standard practice, the dialogues
  generated  by the QGen are used only to compute the loss function,
  and the Guesser is trained by receiving human dialogues. At test time, the model generates a fixed number of questions (5 in our work) and the answers come from the baseline Oracle agent presented in de Vries et al. \shortcite{guesswhat_game}.
Please refer to Shekhar et al. \shortcite{shekhar-etal-2019-beyond} for any additional detail on the model architecture and the training paradigm.

\begin{table}[t]
	\centering
	\begin{tabular}{l|l|l|l|}
		\cline{2-4}
		& \begin{tabular}[c]{@{}l@{}}Human \\ data\end{tabular} & \begin{tabular}[c]{@{}l@{}}Generated \\ data\end{tabular} & \begin{tabular}[c]{@{}l@{}}Mixed \\ (50\%)\end{tabular} \\ \hline
		\multicolumn{1}{|l|}{GRQ} & 0 & 10.3 & 5.4 \\ \hline
		\multicolumn{1}{|l|}{MO} & 0.06 & 0.19 & 0.10 \\ \hline
		\multicolumn{1}{|l|}{Vocab size} & 10469 & 2578 & 4388 \\ \hline
	\end{tabular}
\caption{Features of 3 different training sets. Note that, for human dialogues, the number of tokens occurring at least 3 times is 4900: this forms the vocabulary given to the model.}
\label{tab_intro}
\vspace*{-10pt}
\end{table}
